Bias at a Second Glance: A Deep Dive into Bias for German Educational Peer-Review Data Modeling

Natural Language Processing (NLP) has become increasingly utilized to provide adaptivity in educational applications. However, recent research has highlighted a variety of biases in pre-trained language models. While existing studies investigate bias in different domains, they are limited in addressing fine-grained analysis on educational and multilingual corpora. In this work, we analyze bias across text and through multiple architectures on a corpus of 9,165 German peer-reviews collected from university students over five years. Notably, our corpus includes labels such as helpfulness, quality, and critical aspect ratings from the peer-review recipient as well as demographic attributes. We conduct a Word Embedding Association Test (WEAT) analysis on (1) our collected corpus in connection with the clustered labels, (2) the most common pre-trained German language models (T5, BERT, and GPT-2) and GloVe embeddings, and (3) the language models after fine-tuning on our collected data-set. In contrast to our initial expectations, we found that our collected corpus does not reveal many biases in the co-occurrence analysis or in the GloVe embeddings. However, the pre-trained German language models find substantial conceptual, racial, and gender bias and have significant changes in bias across conceptual and racial axes during fine-tuning on the peer-review data. With our research, we aim to contribute to the fourth UN sustainability goal (quality education) with a novel dataset, an understanding of biases in natural language education data, and the potential harms of not counteracting biases in language models for educational tasks.

==> [COLING 2022] Bias at a Second Glance (1)/tables.tex <==
% \begin{table*}[]
% \resizebox{\textwidth}{!}{
% \begin{tabular}{@{}|r|c|r|r|r|r|lrlr|@{}}
% \toprule
% \multicolumn{1}{|c|}{\textbf{WEAT}} &
%   \textbf{\#} &
%   \multicolumn{1}{c|}{\textbf{Targets}} &
%   \multicolumn{1}{c|}{\textbf{Attributes}} &
%   \textbf{Total} &
%   \textbf{Ratings} &
%   \multicolumn{1}{r}{\textbf{\begin{tabular}[c]{@{}r@{}}Constructive\\ Suggestions\end{tabular}}} &
%   \textbf{\begin{tabular}[c]{@{}r@{}}Critical\\ Aspects\end{tabular}} &
%   \multicolumn{1}{r}{\textbf{Helpful}} &
%   \textbf{\begin{tabular}[c]{@{}r@{}}High\\ Quality\end{tabular}} \\ \midrule
%  &
%   &
%   &
%   &
%   {\color[HTML]{333333} } &
%   \textbf{high} &
%   2.0 &
%   -0.222 &
%   -1.277 &
%   2.0 \\ \cmidrule(l){6-10} 
% \multirow{-2}{*}{Gender} &
%   \multirow{-2}{*}{6} &
%   \multirow{-2}{*}{\begin{tabular}[c]{@{}r@{}}Male vs. \\ Female Names\end{tabular}} &
%   \multirow{-2}{*}{\begin{tabular}[c]{@{}r@{}}Career \\ vs. Family\end{tabular}} &
%   \multirow{-2}{*}{{\color[HTML]{333333} -1.496}} &
%   \textbf{low} &
%   -2.0 &
%   \multicolumn{1}{l}{oov} &
%   2.0 &
%   \multicolumn{1}{l|}{-2.105} \\ \bottomrule
% \end{tabular}}
% \caption{The GloVE models only find one WEAT test with significant effect. We examine the total effect size as well as each of the subsets (high and low scores for constructive suggestions, critical aspects, helpfulness, and quality). oov stands for out-of-vocabulary.}
% \label{tab:glove}
% \end{table*}

% \begin{table}[]
% \small
% \resizebox{0.46\textwidth}{!}{
% \begin{tabular}{@{}|r|c|ccc|ccc|ccc|@{}}
% \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{3}{c}{\textbf{conceptual}} & \multicolumn{3}{c}{\textbf{racial}} & \multicolumn{3}{c}{\textbf{gender}} \\ \midrule
% \textbf{} & \textbf{\#} & \textbf{1} & \textbf{2} & \textbf{9} & \textbf{3} & \textbf{4} & \textbf{5} & \textbf{6} & \textbf{7} & \textbf{8} \\ \midrule
% \textbf{total} & 9165 &  &  & + & + & + & + & + &  &  \\ \midrule
% \multirow{2}{*}{\textbf{quality}} & \multirow{2}{*}{5391} &  &  &  & - & - &  & - &  &  \\
%  &  &  &  & + &  &  & + & + &  &  \\ \midrule
% \multirow{2}{*}{\textbf{critical}} & \multirow{2}{*}{5514} &  &  & - & - & - &  & - &  &  \\
%  &  &  &  &  &  &  & + & + &  &  \\ \midrule
% \multirow{2}{*}{\textbf{helpful}} & \multirow{2}{*}{5886} &  &  & - & - & - &  & - &  &  \\
%  &  &  &  &  &  &  & + & + &  &  \\ \midrule
% \multirow{2}{*}{\textbf{constructive}} & \multirow{2}{*}{5656} &  &  & - & - & - &  & - &  &  \\
%  &  &  &  &  &  &  & + & + &  &  \\ \bottomrule
% \end{tabular}}
% \caption{WEAT co-occurrence analysis across different review rating criteria (quality, critical aspects, helpfulness, constructive) and tests (1-9). $+$ indicates at least one co-occurrence example present in the high ratings for that criteria, and $-$ indicates the same for low ratings. The # column represents the number of positive ratings in these aspects.}
% \label{tab:weat-counts}
% \end{table}

==> tables.tex <==
% \begin{table*}[]
% \resizebox{\textwidth}{!}{
% \begin{tabular}{@{}|r|c|r|r|r|r|lrlr|@{}}
% \toprule
% \multicolumn{1}{|c|}{\textbf{WEAT}} &
%   \textbf{\#} &
%   \multicolumn{1}{c|}{\textbf{Targets}} &
%   \multicolumn{1}{c|}{\textbf{Attributes}} &
%   \textbf{Total} &
%   \textbf{Ratings} &
%   \multicolumn{1}{r}{\textbf{\begin{tabular}[c]{@{}r@{}}Constructive\\ Suggestions\end{tabular}}} &
%   \textbf{\begin{tabular}[c]{@{}r@{}}Critical\\ Aspects\end{tabular}} &
%   \multicolumn{1}{r}{\textbf{Helpful}} &
%   \textbf{\begin{tabular}[c]{@{}r@{}}High\\ Quality\end{tabular}} \\ \midrule
%  &
%   &
%   &
%   &
%   {\color[HTML]{333333} } &
%   \textbf{high} &
%   2.0 &
%   -0.222 &
%   -1.277 &
%   2.0 \\ \cmidrule(l){6-10} 
% \multirow{-2}{*}{Gender} &
%   \multirow{-2}{*}{6} &
%   \multirow{-2}{*}{\begin{tabular}[c]{@{}r@{}}Male vs. \\ Female Names\end{tabular}} &
%   \multirow{-2}{*}{\begin{tabular}[c]{@{}r@{}}Career \\ vs. Family\end{tabular}} &
%   \multirow{-2}{*}{{\color[HTML]{333333} -1.496}} &
%   \textbf{low} &
%   -2.0 &
%   \multicolumn{1}{l}{oov} &
%   2.0 &
%   \multicolumn{1}{l|}{-2.105} \\ \bottomrule
% \end{tabular}}
% \caption{The GloVE models only find one WEAT test with significant effect. We examine the total effect size as well as each of the subsets (high and low scores for constructive suggestions, critical aspects, helpfulness, and quality). oov stands for out-of-vocabulary.}
% \label{tab:glove}
% \end{table*}

% \begin{table}[]
% \small
% \resizebox{0.46\textwidth}{!}{
% \begin{tabular}{@{}|r|c|ccc|ccc|ccc|@{}}
% \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{3}{c}{\textbf{conceptual}} & \multicolumn{3}{c}{\textbf{racial}} & \multicolumn{3}{c}{\textbf{gender}} \\ \midrule
% \textbf{} & \textbf{\#} & \textbf{1} & \textbf{2} & \textbf{9} & \textbf{3} & \textbf{4} & \textbf{5} & \textbf{6} & \textbf{7} & \textbf{8} \\ \midrule
% \textbf{total} & 9165 &  &  & + & + & + & + & + &  &  \\ \midrule
% \multirow{2}{*}{\textbf{quality}} & \multirow{2}{*}{5391} &  &  &  & - & - &  & - &  &  \\
%  &  &  &  & + &  &  & + & + &  &  \\ \midrule
% \multirow{2}{*}{\textbf{critical}} & \multirow{2}{*}{5514} &  &  & - & - & - &  & - &  &  \\
%  &  &  &  &  &  &  & + & + &  &  \\ \midrule
% \multirow{2}{*}{\textbf{helpful}} & \multirow{2}{*}{5886} &  &  & - & - & - &  & - &  &  \\
%  &  &  &  &  &  &  & + & + &  &  \\ \midrule
% \multirow{2}{*}{\textbf{constructive}} & \multirow{2}{*}{5656} &  &  & - & - & - &  & - &  &  \\
%  &  &  &  &  &  &  & + & + &  &  \\ \bottomrule
% \end{tabular}}
% \caption{WEAT co-occurrence analysis across different review rating criteria (quality, critical aspects, helpfulness, constructive) and tests (1-9). $+$ indicates at least one co-occurrence example present in the high ratings for that criteria, and $-$ indicates the same for low ratings. The # column represents the number of positive ratings in these aspects.}
% \label{tab:weat-counts}
% \end{table}
